DART: An AIGT Detector using AMR of Rephrased Text

As large language models (LLMs) generate more human-like texts, concerns about the side effects of AI-generated texts (AIGT) have grown. So, researchers have developed methods for detecting AIGT. However, two challenges remain. First, the performance of detecting black-box LLMs is low because existing models focus on probabilistic features. Second, most AIGT detectors have been tested on a single-candidate setting, which assumes that we know the origin of an AIGT and which may deviate from the real-world scenario. To resolve these challenges, we propose DART, which consists of four steps: rephrasing, semantic parsing, scoring, and multiclass classification. We conducted three experiments to test the performance of DART. The experimental result shows that DART can discriminate multiple black-box LLMs without probabilistic features and the origin of AIGT.

==> tables/tab-statistics-total.tex <==


% \begin{tabular}{@{}l@{\;}r@{\;}|@{\;}r@{\;\;}r@{\;\;}r@{\;\;}r@{\;\;}r@{}}
% \toprule
%                       &  Mac.           & \multicolumn{2}{c}{\small GPT series}     & {\small Llama}            & {\small Gemini} & {\small Human}\\ 
%                       & F1             & { 3.5T}     & { 4o}            & { 3}            & { 1.5 F}      &  \\ 
% \midrule
% SeqXGPT               & xxx.x                                 & xxx.x                        & xxx.x                                 & xxx.x                                 & xxx.x                                 &xxx.x                                 \\
% \midrule
% DART\textsubscript{SVM}            & xxx.x                                 & xxx.x                                 & xxx.x                                 & xxx.x                                 & xxx.x                                 &xxx.x                                 \\
% \phantom{DART}\textsubscript{DT}             & \textbf{xxx.x} & { \textbf{xxx.x}}          & { \textbf{xxx.x}} & { \textbf{xxx.x}} & { \textbf{xxx.x}} &{\textbf{xxx.x}}\\ 
% \bottomrule
% \end{tabular}%
% % }
% \caption{Results of multi-candidate experiment}
% \label{tab:multi-model result2}
% \end{table}



\begin{table} %[!htp]
\centering
\begin{tabular}{@{}@{\;\;}lrrl}
\toprule
        & \multicolumn{1}{l}{\# chars}    & \multicolumn{1}{l}{\#    tokens} & \# sample                \\
\midrule       
Human         & 1541.5                              & 311.8                            & \multicolumn{1}{r}{3989}  \\
LLMs     & 818.2                             & 185.8                           & \multicolumn{1}{r}{15956} \\
% \quad GPT-3.5T            & xxx.x                              & xxx.x                            & \multicolumn{1}{r}{3989}  \\
% \quad GPT-4o            & xxx.x                             & xxx.x                           &                          \\
% \quad Llama 3            & xxx.x                             & xxx.x                           &                          \\
% \quad Gemini-1.5F         & xxx.x                             & xxx.x                           &                          \\
\bottomrule
\end{tabular}
\caption{Statistics of collected datasets}
\label{tab:statistics}
\end{table}

==> tables/tab2-result.tex <==
\begin{table} %[!htp]
\centering
% \resizebox{\textwidth}{!}{%
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{@{\;}l@{\;\;}r|r@{\;\;}r@{\;\;}r@{\;\;}r@{\;}}
\toprule
                      &                 & \multicolumn{2}{c}{\small GPT series}     & {\small Llama}            & {\small Gemini} \\ 
                      & Avg             & { 3.5T}     & { 4o}            & { 3}            & { 1.5 F}        \\ 
\midrule
DetectGPT             & 65.8                                     & 65.8& 65.6& 65.8                                 & 65.7\\
f-DetectGPT        & 60.1                                     & 58.0                                 & 66.2                                 & 62.4                                 & 53.8                                 \\
DNA-GPT               & 54.1                                     & 56.6                                 & 57.4                                 & 54.8                                 & 47.7                                 \\
% Roberta-base          & 77.4                                     & 77.0                                 & 78.5                                 & 77.4                                 & 76.8                        \\
Roberta-base        & 77.2& 76.8& 80.0& 74.7& 77.1\\
SeqXGPT               & 54.1                                     & 86.5                                 & 45.9                                 & 41.6                                 & 42.3                                 \\
\midrule
DART\textsubscript{SVM}            & 82.8                                     & { 87.1}          & { 86.1}          & 84.8                                 & { 73.3}          \\
\phantom{DART}\textsubscript{DT}             & \textbf{96.5}                                     & { \textbf{100.0}} & { \textbf{88.1}} & { \textbf{100.0}} & { \textbf{97.9}} \\ 
\bottomrule
\end{tabular}%
% }
\caption{Results of single-candidate experiment}
\label{tab:xxx}
\end{table}

\begin{table} %[!htp]
\centering
% \resizebox{\textwidth}{!}{%
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{@{}l@{\;}r@{\;}|@{\;}r@{\;\;}r@{\;\;}r@{\;\;}r@{\;\;}r@{}}
\toprule
                      &  Mac.           & \multicolumn{2}{c}{\small GPT series}     & {\small Llama}            & {\small Gemini} & {\small Human}\\ 
                      & F1             & { 3.5T}     & { 4o}            & { 3}            & { 1.5 F}      &  \\ 
\midrule
SeqXGPT               & 59.2                                 & 54.3                        & 66.4                                 & 44.8                                 & 61.4                                 &69.3                                 \\
\midrule
DART\textsubscript{SVM}            & 65.0                                 & 67.4                                 & 71.0                                 & 54.0                                 & 67.0                                 &65.4                                 \\
\phantom{DART}\textsubscript{DT}             & \textbf{81.2} & { \textbf{80.6}}          & { \textbf{76.6}} & { \textbf{85.8}} & { \textbf{85.5}} &{\textbf{77.3}}\\ 
\bottomrule
\end{tabular}%
% }
\caption{Results of multi-candidate experiment}
\label{tab:xxx}
\end{table}

